PromptWise: Online Learning for Cost-Aware Prompt Assignment in Generative Models

The rapid advancement of generative AI has provided users with a wide range of well-trained models to address diverse prompts. When selecting a model for a given prompt, users should weigh not only its performance but also its service cost. However, existing model-selection methods typically emphasize performance while overlooking cost differences. In this paper, we introduce PromptWise, an online learning framework that assigns prompts to generative models in a cost-aware manner. PromptWise estimates prompt-model compatibility to select the least expensive model expected to deliver satisfactory outputs. Unlike standard contextual bandits that make a one-shot decision per prompt, PromptWise employs a cost-aware bandit structure that allows sequential model assignments per prompt to reduce total service cost. Through numerical experiments on tasks such as code generation and translation, we demonstrate that PromptWise can achieve performance comparable to baseline selection methods while incurring substantially lower costs. The code is available at: github.com/yannxiaoyanhu/PromptWise.

==> draft.tex <==
\noindent\textbf{Average-reward criterion.}\quad Consider $f(\{r_{t,i}\}_{i=1}^{\tau_t}) = \tau_t^{-1} \sum_{i=1}^{\tau_t} r_{t,i} $ and $\tau_{\max} < \infty$, where the random reward of arm $a \in \gA$ is drawn from a Bernoulli distribution denoted by $\Ber(\nu_a(x))$. The average-reward criterion suits a scenario where the goal is to pass a ``test''. Solving the oracle policy can be formulated as an episodic Markov Decision Process~(MDP) and hence solved by dynamic programming (DP). Details can be found in Appendix~\ref{sec: a.2}.

\begin{assumption}[Average-reward criterion]
\label{aspt-4.2}
For any action $a \in \gA$, there exists $\theta_a^\star \in \sR^d$ such that $\nu_a(x) = \mu(\langle \theta_a^\star, x \rangle)$ for any context $x \in \gX \subset \sR^d$.
\end{assumption}

\subsection{Average-Reward Oracle}
\label{sec: a.2}

\begin{proof}
Fix a context $x$ and rewrite $\nu_a := \nu_a(x)$ for convenience. The problem can be formulated as an episodic MDP with states $\gS = \overline{[\tau_{\max}]} \cup \{\gT\}$ and horizon $\tau_{\max}$, where $\gT$ is the terminal state and $\overline{[\tau_{\max}]} := \{0\} \cup [\tau_{\max}] = \{0,1, \cdots, \tau_{\max} \}$ indicates the total reward $\sum_{n=1}^i r_{t, i}$ up to the current round. The transition kernel at the $i$-th round is given by
\begin{equation*}
    P_i(n' | n, a) = 
    \begin{cases}
        \nu_a, & \text{if } n' = n + 1, \\
        1 - \nu_a, & \text{if } n' = n,
    \end{cases}
    \quad \textup{and}\quad
    P_i(\gT | n, a_0) = 1
\end{equation*}
The reward function is defined as $r_i(n,a,n') = u_{i+1}(n') - u_i(n) - \lambda c_a$ and $r_i(n,a_0,\gT) = 0$, where $u_i(n)=\bm{1}[\frac{n}{i} \ge \alpha]$ for any $(n,i) \in [\tau_{\max}] \times [\tau_{\max}]$. Hence, the oracle policy admits the Bellman optimality equation:
\begin{equation*}
\label{eq-39}
\begin{aligned}
    V_i^\star(n) = \max\Bigg\{0, \max_{a \in \gA} \Big\{& \nu_a \left(u_{i+1}(n+1) - u_i(n) - \lambda c_a + V_{i+1}^\star(n+1)\right) \\
    & + (1 - \nu_a) \left( u_{i+1}(n) - u_i(n) - \lambda c_a + V_{i+1}^\star(n) \right)\Big\} \Bigg\},
\end{aligned}
\end{equation*}
where $V_{\tau_{\max} + 1}^\star(\cdot) = 0$.
\end{proof}


For the average-reward criterion, let $\hatnu_a(x) \ge \nu_a(x)$ for any action $a \in \gA$ and context $x \in \gX$. Recall that $\overline{[\tau_{\max}]} = \{0,1,\cdots,\tau_{\max}\}$. Next, we show that $\hatV_i(n) - V^\star_i(n) \ge (\tau_{\max} - i)(\hatnu_a(x) - \nu_a(x))$ for any $(i,n) \in [\tau_{\max}] \times \overline{[\tau_{\max}]}$ by induction, where $\hatV_i(\cdot)$ is the (pseudo-)value obtained by the optimal policy on $\{\hatnu_a(x): a \in \gA\}$ and $V^\star_i(\cdot)$ is defined in Equation~(\ref{eq-39}). First, we have $\hatV_{\tau_{\max} + 1}(\cdot) = 0 \ge V_{\tau_{\max} + 1}^\star(\cdot)$. Assume the argument holds for round $i \in [\tau_{\max}]$ and $i \ge 2$. Then, we have
\begin{equation*}
\begin{aligned}
    \hatV_i(n) = \max\left\{0, \max_{a \in \gA} \widehat{Q}_i(n,a) \right\},
\end{aligned}
\end{equation*}
where
\begin{equation*}
    \widehat{Q}_i(n,a) := \hatnu_a(x) \left(u_{i+1}(n+1) + \hatV_{i+1}(n+1)\right) + (1 - \hatnu_a(x)) \left( u_{i+1}(n) + \hatV_{i+1}(n) \right) - u_i(n) - \lambda c_a
\end{equation*}
Note that for any $a \in \gA$, we have
\begin{align*}
    & \widehat{Q}_i(n,a) - Q^\star_i(n,a) \\
    = & \left(\hatnu_a(x) - \nu_a(x)\right) \left(u_{i+1}(n+1) + \hatV_{i+1}(n+1)\right) + \nu_a(x) \left(\hatV_{i+1}(n+1) - V^\star_{i+1}(n+1) \right) \\
    & + (\nu_a(x) - \hatnu_a(x)) \left( u_{i+1}(n) + \hatV_{i+1}(n) \right) + (1 - \nu_a(x)) \left(\hatV_{i+1}(n) - V^\star_{i+1}(n) \right) \\
    \ge & (\hatnu_a(x) - \nu_a(x)) \left(u_{i+1}(n+1) + \hatV_{i+1}(n+1) - u_{i+1}(n) - \hatV_{i+1}(n)\right) \\
    \ge & 0
\end{align*}
where the last inequality holds by $u_{i+1}(n+1) \ge u_{i+1}(n)$ and $\hatV_{i+1}(n+1) \ge \hatV_{i+1}(n)$. We conclude the proof.

\begin{theorem}[Average-reward]
\label{thm-reg-dec-avg}

Let $\{ \hatnu_a(x) \in [0,1]: a \in \gA \}$ denote any estimation of $\{ \nu_a(x): a \in \gA \}$ for some context $x \in \gX$. Consider any policy $\pi: [\tau_{\max}] \times \overline{[\tau_{\max}]} \to \Bar{\gA}$, i.e., the policy takes action $\pi_i(n)$ at the $i$-th round given a cumulative reward of $n$. We have $\hatu^{\pi,\textup{avg}}(x) - u^{\pi,\textup{avg}}(x) \le \tau_{\max} \cdot \max_{a \in \gA} |\hatnu(x) - \nu_a(x)|$.

\begin{proof}
Consider any deterministic policy $\pi: [\tau_{\max}] \times \overline{[\tau_{\max}]} \to \Bar{\gA}$. For any $(i,n)$ pair where $\pi_i(n) = a_0$, we have $\hatV_i^\pi(n) = V_i^\pi(n) = 0$. In the following, we assume $\pi_i(n) \in \gA$. For convenience, we fix a context $x$ and rewrite $\hatnu_{a} := \hatnu_{a}(x)$ and $\nu_a := \nu_a(x)$. We have
\begin{align*}
    & \hatV^\pi_i(n) - V^\pi_i(n) \\
    = & \left( \hatnu_a - \nu_a \right) \left(u_{i+1}(n+1) + \hatV_{i+1}^\pi(n+1)\right) + \nu_a \left(\hatV_{i+1}^\pi(n+1) - V^\pi_{i+1}(n+1) \right) \\
    & + (\nu_a - \hatnu_a) \left( u_{i+1}(n) + \hatV_{i+1}^\pi(n) \right) + (1 - \nu_a) \left(\hatV_{i+1}^\pi(n) - V^\pi_{i+1}(n) \right) \\
    \le & |\nu_a - \hatnu_a| + \E \left[ \hatV_{i+1}^\pi(\cdot) - V^\pi_{i+1}(\cdot) \right] \\
    \le & (\tau_{\max} - i + 1) \cdot \max_{a \in \gA} |\nu_a - \hatnu_a|,
\end{align*}
which concludes the proof.
\end{proof}
\end{theorem}


